Learning Representations for Counterfactual Inference

Observational studies are rising in importance due to the widespread accumulation of data in fields such as healthcare, education, employment and ecology. We consider the task of answering counterfactual questions such as, "Would this patient have lower blood sugar had she received a different medication?". We propose a new algorithmic framework for counterfactual inference which brings together ideas from domain adaptation and representation learning. In addition to a theoretical justification, we perform an empirical comparison with previous approaches to causal inference from observational data. Our deep learning algorithm significantly outperforms the previous state-of-the-art.

==> fig_model.tex <==

\def\layersep{1.8cm}
\begin{tikzpicture}[->,>=latex,shorten >=1pt, thick,draw=black!50, node distance=\layersep]

    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{box}=[rectangle,minimum width=1.0cm,minimum height=1.0cm,draw=black!50];
    \tikzstyle{noline}=[box, fill=black!0, minimum width=0.6cm,minimum height=0.6cm, draw=black!0]];
    %\tikzstyle{input neuron}=[box, fill=green!15];

    % Draw the representation node
    \node[noline] (input) at (0,0) {$\bx$};
    \node[box, right of=input] (transform) {$g(\cdot)$};
    \node[noline, right of=transform] (rep) {$\phi$};
    \node[noline, below of=input] (group) {$t$};
    \node[noline, right of=rep] (output) {$\hat{\by}$};
    \node[noline, below of=output] (dist) {$\imb(\phi_C, \phi_T)$};
    %\node[hidden neuron] (lstm-1) at (\layersep,0) {$\bc_0$};
    %\node[output neuron, above of=lstm-1] (output-1) {$\bh_0$};

    \path (input) edge (transform);
    \path (transform) edge (rep);
    \path (rep) edge (output);
    \path (rep) edge (dist);
    \path (group) edge (output);
    \path (group) edge (dist);
    \path (group) edge (transform);
\end{tikzpicture}

